Dissipation properties of transport noise in the two-layer quasi-geostrophic model

A stochastic version of the two-layer quasi-geostrophic model (2LQG) with multiplicative transport noise is analysed. This popular intermediate complexity model describes large scale atmosphere and ocean dynamics at the mid-latitudes. The transport noise, which acts on both layers, accounts for the unresolved small scales. After establishing the well-posedness of the perturbed equations, we show that, under a suitable scaling of the noise, the solutions converge to the deterministic 2LQG model with enhanced dissipation. Moreover, these solutions converge to the deterministic stationary ones on the long time horizon.

==> preamble.tex <==
\usepackage[english]{babel}

% \usepackage{layout} % package to show layout with command \layout
% \usepackage{showframe} % show the layout on every page of the document
% \usepackage{geometry}
% \geometry{
%  a4paper,
%  total={150mm,230mm},
%  left=30mm,
%  % right=25mm,
%  top=30mm,
%  % bottom=25mm
%  }
% 35 pages = 25 pages template AnnalsAppliedProbability ~ cut to 25-30 pages

\RequirePackage[a4paper,top=2.54cm,bottom=2.54cm,left=1.90cm,right=1.90cm,%
                headsep=1em,includehead,includefoot]{geometry}

\usepackage{amsmath,amsthm,amsfonts,amssymb,bm}
\usepackage{mathtools}
\usepackage{hyperref} % fancy references 
\usepackage{url}
\usepackage{breakcites}
\usepackage{bbm} % for boldface maths \bm
\usepackage{graphicx,subfigure,caption, float}
\usepackage{array}
\usepackage{color} % for colored text
\usepackage{colortbl}
\usepackage{newlfont}
\usepackage{mathrsfs}
\usepackage{lineno} % for the line numbers
\usepackage[toc,page]{appendix}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{physics}
\usepackage{fancyhdr}
% \usepackage{scrtime} % to show the time of compilation
\usepackage{enumitem}
\usepackage{multirow}
\renewcommand{\arraystretch}{1.35}

\usepackage{crossreftools} %for personalised item label referenc   % comment out in TexMaker
\usepackage{apptools}

% \usepackage[style=alphabetic, giveninits=true]{biblatex}
% \addbibresource{Biblio_phd.bib}
 
\addto\extrasenglish{\def\subsectionautorefname{Section}} %
\addto\extrasenglish{\def\sectionautorefname{Section}} %to have subsections called sections in ref

\usepackage{aliascnt}
\pgfplotsset{compat=1.16}   % comment out in TexMaker
% \linespread{1.2}


\theoremstyle{plain}
\newtheorem{thrm}{Theorem}
    \newtheorem{theorem}{Theorem}[section]
    \newaliascnt{corollary}{theorem}
    \newtheorem{thmmanual}{Theorem}[section]
    \newtheorem{corollary}[corollary]{Corollary}
    \aliascntresetthe{corollary}
    \newcommand{\corollaryautorefname}{Corollary}
    
    \newaliascnt{lemma}{theorem}
    \newtheorem{lemma}[lemma]{Lemma}
    \aliascntresetthe{lemma}
    \newcommand{\lemmaautorefname}{Lemma}
    
    \newaliascnt{proposition}{theorem}
    \newtheorem{proposition}[proposition]{Proposition}
    \aliascntresetthe{proposition}
    \newcommand{\propositionautorefname}{Proposition}
    
    \newtheorem{assum}{Assumption}
    \newcommand{\assumautorefname}{Assumption}

\theoremstyle{definition}
    \newaliascnt{definition}{theorem}
    \newtheorem{definition}[definition]{Definition}
    \aliascntresetthe{definition}
    \newcommand{\definitionautorefname}{Definition}
    
    % \newaliascnt{assumption}{theorem}
    % \newtheorem{assumption}[assumption]{Assumption}
    % % \newtheorem*{assumptionA}{Assumption A}
    % \aliascntresetthe{assumption}
    % \newcommand{\assumptionautorefname}{Assumption}

\theoremstyle{remark}
    \newaliascnt{remark}{theorem}
    \newtheorem{remark}[remark]{Remark}
    \aliascntresetthe{remark}
    \newcommand{\remarkautorefname}{Remark}
    
 \newaliascnt{example}{theorem}
    \newtheorem{example}[example]{Example}
    \aliascntresetthe{example}
    \newcommand{\exampleautorefname}{Example}
    
% \newtheorem*{assumption*}{\assumptionnumber}
% \providecommand{\assumptionnumber}{}
% \makeatletter
% \newenvironment{assumption}[1]
%  {%
%   \renewcommand{\assumptionnumber}{Assumption #1}%
%   \begin{assumption*}%
%   \protected@edef\@currentlabel{#1}%
%  }
%  {%
%   \end{assumption*}
%  }
% \makeatother
%
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cF}{\mathcal{F}}

\newcommand{\tq}{\tilde{\mathbf{q}}}
\newcommand{\tpsi}{\Tilde{\bm{\psi}}}
\newcommand{\td}{\tilde{d}}
\newcommand{\tY}{\tilde{Y}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tA}{\tilde{A}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tcO}{\tilde{\cO}}
\newcommand{\teta}{\tilde{\eta}}

\newcommand{\q}{\mathbf{q}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\bm{w}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfphi}{\bm{\phi}}
\newcommand{\bfpsi}{\bm{\psi}}
\newcommand{\bfeta}{\bm{\eta}}
\newcommand{\bfxi}{\bm{\xi}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\Hmo}{\mathbf{H}^{-1}} % NEW!!!!!!!!!!!!
\newcommand{\Ltwo}{\mathbb{L}^2}
\newcommand{\bLtwo}{\mathbf{L}^2}
\newcommand{\Ho}{\mathbf{H}^1}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\Cd}{\mathcal{C}_{\tilde{d}}}
\newcommand{\CU}{\mathcal{C}_U}

\newcommand{\oPi}{\Pi^\perp}
\newcommand{\Wtd}[2]{W_{\tilde{d}}\left( #1, #2 \right)}

\newcommand{\Lip}[1]{\operatorname{Lip}_d \left( {#1} \right)}
\newcommand{\Lipt}[1]{\operatorname{Lip}_{\tilde{d}} \left( {#1} \right)}
\newcommand{\lip}{\operatorname{Lip}}

\newcommand{\fa}{\quad \text{for all }\,}
\newcommand{\quand}{\quad \text{and} \quad }
\newcommand{\as}{\quad \bP\text{--a.s.}}
\newcommand{\Ieps}{I_{\varepsilon}}
% \DeclareMathOperator{\ker}{ker}
\newcommand{\scp}[1]{{\left\langle #1 \right\rangle}}

\DeclareMathOperator{\cls}{cls}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\Law}{Law}

\newcommand{\ddt}{\tfrac{\text{d}}{\text{d}t}}

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

    
    
\hyphenation{di-men-sion-al}
\hyphenation{se-mi-group}
\hyphenation{geo-stro-phic}
\hyphenation{bound-ed}
\hyphenation{mod-el}
\hyphenation{neigh-bor-hood}
    
% \usepackage{tridelim}
% \DeclarePairedDelimiter{\tripleparen}{\lPparen}{\rPparen}


% This is put into the margin
\newcommand{\comment}[2]{{\color{red}$^*$\marginpar{\color{red}\flushleft\ttfamily\small #1 says:\color{black} #2}\color{black} }}
% To mark new material, use \ins{<Your initials>} Blablabla \off{{Your initials}}
% To mark material for deletion, use \del{<Your initials>} Blablabla \off{{Your initials}}
\newcommand{\ins}{\color{blue}}
\newcommand{\del}{\color{red}}
\newcommand{\off}{\color{black}}
\newcommand{\rmk}[1]{{\color{red}\ttfamily #1}}

%% % The following are draft options
%
%  \usepackage{showlabels}
%  \renewcommand{\showlabelfont}{\tiny}
%  \linenumbers
 
% \usepackage{fancyhdr}
% \usepackage[realmainfile]{currfile}

% \usepackage[12hr]{datetime} 
% \fancypagestyle{plain}{
% \fancyhf{}
% \rfoot{\texttt{Compiled on {\ddmmyyyydate\today} at \currenttime}}
% \lfoot{\texttt{Page \thepage}}
% % \chead{\texttt{\currfilename}}
% \renewcommand{\headrulewidth}{0pt}
% }
% \pagestyle{plain}

% 
% \setlength{\hoffset}{-1in}
% \setlength{\oddsidemargin}{2cm}
% \setlength{\textwidth}{11cm}
% \setlength{\voffset}{-1in}
% \setlength{\topmargin}{2.5cm}
% \setlength{\topskip}{0cm}
% \setlength{\headheight}{0cm}
% \setlength{\headsep}{0cm}
% \setlength{\textheight}{24cm}
% \setlength{\marginparwidth}{6cm}
%% % end of draft options


%% The following are LATEXDIFF definitions
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

%% end Latexdiff definitions


\newcommand{\footremember}[2]{%
    \footnote{#2}
    \newcounter{#1}
    \setcounter{#1}{\value{footnote}}%
}
\newcommand{\footrecall}[1]{%
    \footnotemark[\value{#1}]%
} 


